Global-Local Face Upsampling Network

Face hallucination, which is the task of generating a high-resolution face image from a low-resolution input image, is a well-studied problem that is useful in widespread application areas. Face hallucination is particularly challenging when the input face resolution is very low (e.g., 10 x 12 pixels) and/or the image is captured in an uncontrolled setting with large pose and illumination variations. In this paper, we revisit the algorithm introduced in [1] and present a deep interpretation of this framework that achieves state-of-the-art under such challenging scenarios. In our deep network architecture the global and local constraints that define a face can be efficiently modeled and learned end-to-end using training data. Conceptually our network design can be partitioned into two sub-networks: the first one implements the holistic face reconstruction according to global constraints, and the second one enhances face-specific details and enforces local patch statistics. We optimize the deep network using a new loss function for super-resolution that combines reconstruction error with a learned face quality measure in adversarial setting, producing improved visual results. We conduct extensive experiments in both controlled and uncontrolled setups and show that our algorithm improves the state of the art both numerically and visually.

==> Figures/Adversarial/32/adversarial32.tex <==
\begin{tabular}[t]{ccccc}
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Input_00343.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/MS_00343.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad1_00343.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad2_00343.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/GT_00343.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Input_00307.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/MS_00307.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad1_00307.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad2_00307.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/GT_00307.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Input_00212.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/MS_00212.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad1_00212.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad2_00212.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/GT_00212.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Input_00263.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/MS_00263.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad1_00263.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad2_00263.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/GT_00263.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Input_00314.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/MS_00314.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad1_00314.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad2_00314.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/GT_00314.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Input_00500.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/MS_00500.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad1_00500.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad2_00500.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/GT_00500.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Input_00519.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/MS_00519.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad1_00519.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad2_00519.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/GT_00519.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Input_01345.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/MS_01345.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad1_01345.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad2_01345.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/GT_01345.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Input_00733.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/MS_00733.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad1_00733.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad2_00733.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/GT_00733.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Input_00832.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/MS_00832.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad1_00832.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad2_00832.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/GT_00832.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Input_01080.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/MS_01080.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad1_01080.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad2_01080.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/GT_01080.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Input_00207.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/MS_00207.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad1_00207.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/Ad2_00207.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Adverserial/32/GT_00207.png}\\ 
\end{tabular}

==> Figures/Color/16/color16.tex <==
\begin{tabular}[t]{ccccc}
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Input_00078.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Cubic_00078.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Rec_00078.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Ad_00078.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/GT_00078.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Input_00125.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Cubic_00125.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Rec_00125.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Ad_00125.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/GT_00125.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Input_00140.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Cubic_00140.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Rec_00140.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Ad_00140.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/GT_00140.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Input_00114.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Cubic_00114.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Rec_00114.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Ad_00114.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/GT_00114.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Input_00092.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Cubic_00092.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Rec_00092.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Ad_00092.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/GT_00092.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Input_00188.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Cubic_00188.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Rec_00188.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/Ad_00188.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/16/GT_00188.png}\\ 
\end{tabular}

==> Figures/Color/32/color32.tex <==
\begin{tabular}[t]{ccccc}
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Input_00001.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Cubic_00001.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Rec_00001.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Ad_00001.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/GT_00001.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Input_00005.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Cubic_00005.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Rec_00005.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Ad_00005.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/GT_00005.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Input_00007.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Cubic_00007.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Rec_00007.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Ad_00007.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/GT_00007.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Input_00012.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Cubic_00012.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Rec_00012.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Ad_00012.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/GT_00012.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Input_00058.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Cubic_00058.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Rec_00058.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Ad_00058.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/GT_00058.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Input_00083.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Cubic_00083.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Rec_00083.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/Ad_00083.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Color/32/GT_00083.png}\\ 
\end{tabular}

==> Figures/Failure/16/failure16.tex <==
\begin{tabular}[t]{cccc}
\includegraphics[width=0.18\textwidth]{Figures/Failure/16/Input_00188.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/16/Cubic_00188.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/16/GLN_00188.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/16/GT_00188.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Failure/16/Input_01072.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/16/Cubic_01072.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/16/GLN_01072.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/16/GT_01072.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Failure/16/Input_01181.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/16/Cubic_01181.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/16/GLN_01181.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/16/GT_01181.png}\\ 
\end{tabular}

==> Figures/Failure/32/failure32.tex <==
\begin{tabular}[t]{cccc}
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/Input_01181.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/Cubic_01181.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/GLN_01181.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/GT_01181.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/Input_01140.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/Cubic_01140.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/GLN_01140.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/GT_01140.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/Input_00381.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/Cubic_00381.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/GLN_00381.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/GT_00381.png}\\ 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/Input_00154.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/Cubic_00154.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/GLN_00154.png}& 
\includegraphics[width=0.18\textwidth]{Figures/Failure/32/GT_00154.png}\\ 
\end{tabular}
